All AI Models are Wrong, but Some are Optimal

AI models that predict the future behavior of a system (a.k.a. predictive AI models) are central to intelligent decision-making. However, decision-making using predictive AI models often results in suboptimal performance. This is primarily because AI models are typically constructed to best fit the data, and hence to predict the most likely future rather than to enable high-performance decision-making. The hope that such prediction enables high-performance decisions is neither guaranteed in theory nor established in practice. In fact, there is increasing empirical evidence that predictive models must be tailored to decision-making objectives for performance. In this paper, we establish formal (necessary and sufficient) conditions that a predictive model (AI-based or not) must satisfy for a decision-making policy established using that model to be optimal. We then discuss their implications for building predictive AI models for sequential decision-making.

==> Figures/DT_classes/mutistep.tex <==
\begin{tikzpicture}[
    process/.style={circle, draw, fill=blue!20, minimum size=2mm, inner sep=1pt, font=\small},
    groundtruth/.style={draw=black, thick},
    singlesim/.style={draw=black, thick, densely dashed},
    multisim/.style={draw=black, thick, densely dotted},
    arrow/.style={-{Latex[length=2mm, width=2mm]}, thick},
    label/.style={font=\footnotesize, inner sep=2pt}
]

% Draw the true trajectory as a reference (from s0 to s10)
\draw[groundtruth] (0, 0) -- (10, 0);

% Denote time steps along the true trajectory
\foreach \i in {0,1,...,10} {
    \ifnum\i=0
        \node[anchor=north] at (\i, 0) {$\vect{s}_t$};
    \else
        \node[anchor=north] at (\i, 0) {$\vect{s}_{t+\i}$};
    \fi
}

% Single-step Digital Twin points with less divergence
\foreach \i in {0,1,...,9} {
    \node[process] (s\i) at (\i, {0.05 * \i * \i - 0.1 * \i}) {};
    \ifnum\i>0
        \draw[singlesim] (s\the\numexpr\i-1\relax) -- (s\i);
    \fi
}

% Multi-step Digital Twin with divergence in the same direction, starting from the same point
\draw[multisim] (0, 0) .. controls (3, 0.5) and (7, 1) .. (10, 1.5);

% Add a legend
\begin{scope}[shift={(0, 3)}] % Adjust this shift for better positioning of the legend
    \draw[groundtruth] (0, 0) -- (1, 0) node[right] {True Trajectory};
    \draw[singlesim] (0, -0.5) -- (1, -0.5) node[right] {Single-Step Predictions};
    \draw[multisim] (0, -1) -- (1, -1) node[right] {Multi-Step Prediction};
\end{scope}

\end{tikzpicture}


==> Figures/Estimation/figure.tex <==
\begin{tikzpicture}[
    every node/.style={font=\sffamily},
    align=center
]

% Define positions
\node[inner sep=0pt] (physical) at (0, 0) {\includegraphics[width=3cm]{/home/akhil/PostDoc/Digital Twin/Paper/Digital-Twin/paper/Figures/Estimaton/physical_twin.jpg}};
\node[below=0.2cm of physical] {Physical Twin};

\node[inner sep=0pt] (digital) at (6, 0) {\includegraphics[width=3cm]{digital_twin.jpg}};
\node[below=0.2cm of digital] {Digital Twin};

\node[inner sep=0pt] (data) at (3, -2.5) {\includegraphics[width=2.5cm]{data.jpg}};
\node[below=0.2cm of data] {Data};

\node[inner sep=0pt] (estimation) at (3, 2) {\includegraphics[width=2.5cm]{estimation_methods.jpg}};
\node[above=0.2cm of estimation] {Estimation Methods};

% Arrows for flow
\draw[->, thick] (physical) -- node[above] {Measurements} (data);
\draw[->, thick] (data) -- node[above] {Estimation} (estimation);
\draw[->, thick] (estimation) -- (digital);
\draw[<->, thick] (physical) -- node[above] {} (digital);

% Add formula near digital twin
\node[align=center] at (6, -2.5) {
    $J = \mathbb{E}\left[\sum_{k=0}^\infty \gamma^k L\left(\vect{s}_k, \vect{a}_k\right)\right]$
};

\end{tikzpicture}

==> Figures/Estimation/plot.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\columnwidth, % Adjust to fit in a single column
        height=6cm, % You can change this to adjust the aspect ratio
        xlabel={$\phi$},
        ylabel={$\rho (\phi)$},
        %title={Bayesian Update with Flatter Prior, Likelihood, and Posterior},
        legend pos=north east,
        legend style={font=\small, draw=none},
        grid=none
    ]

    % Plot Prior
    \addplot[
        black, loosely dashed
    ] table [x=x, y=prior, col sep=comma] {Figures/Estimation//bayesian_update_data.csv};
    \addlegendentry{prior}

    % Plot Likelihood
    \addplot[
        black, thin
    ] table [x=x, y=likelihood, col sep=comma] {Figures/Estimation/bayesian_update_data.csv};
    \addlegendentry{\ac{mle}}

    % Plot Posterior
    \addplot[
        black, dash pattern=on 4pt off 2pt on 1pt off 2pt
    ] table [x=x, y=posterior, col sep=comma] {Figures/Estimation/bayesian_update_data.csv};
    \addlegendentry{\ac{map}}

    % Vertical line for Expectation
    \addplot[
        black, densely dotted, thick
    ] coordinates {(1, 0) (1, 0.8)};
    \addlegendentry{$\mathbb{E}$}

    \end{axis}
\end{tikzpicture}

==> Figures/house/plot.tex <==
\begin{tikzpicture}
    \matrix[
        column sep=0.5cm, % Space between columns
        row sep=0.5cm, % Space between rows
        align=center
    ] {
        % First row, first column (Price for N1d_H6h)
        \begin{axis}[
            width=0.45\textwidth,
            height=0.2\textwidth,
            ylabel={Price},
            xmin=0, xmax=30,
            xtick={0,5,10,15,20,25,30},
            legend pos=north east,
            grid=major,
            legend style={draw=none},
            title={N1d H6h}
        ]
            \addplot[
                color=blue, thick
            ] table [
                x expr=\coordindex, 
                y=mean_price, 
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};
            
            \addplot [
                name path=upper, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_price} + sqrt(\thisrow{var_price}),
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};

            \addplot [
                name path=lower, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_price} - sqrt(\thisrow{var_price}),
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};

            \addplot[blue!50, fill opacity=0.2] fill between[of=upper and lower];
        \end{axis}
        &
        % First row, second column (Price for N1d_H12h)
        \begin{axis}[
            width=0.45\textwidth,
            height=0.2\textwidth,
            ylabel={Price},
            xmin=0, xmax=30,
            xtick={0,5,10,15,20,25,30},
            legend pos=north east,
            grid=major,
            legend style={draw=none},
            title={N1d H12h}
        ]
            \addplot[
                color=blue, thick
            ] table [
                x expr=\coordindex, 
                y=mean_price, 
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};
            
            \addplot [
                name path=upper, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_price} + sqrt(\thisrow{var_price}),
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};

            \addplot [
                name path=lower, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_price} - sqrt(\thisrow{var_price}),
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};

            \addplot[blue!50, fill opacity=0.2] fill between[of=upper and lower];
        \end{axis}
        \\
        % Second row, first column (Comfort for N1d_H6h)
        \begin{axis}[
            width=0.45\textwidth,
            height=0.2\textwidth,
            ylabel={Comfort},
            xmin=0, xmax=30,
            xtick={0,5,10,15,20,25,30},
            legend pos=north east,
            grid=major,
            legend style={draw=none},
        ]
            \addplot[
                color=green, thick
            ] table [
                x expr=\coordindex, 
                y=mean_comfort, 
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};
            
            \addplot [
                name path=upper, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_comfort} + sqrt(\thisrow{var_comfort}),
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};

            \addplot [
                name path=lower, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_comfort} - sqrt(\thisrow{var_comfort}),
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};

            \addplot[green!50, fill opacity=0.2] fill between[of=upper and lower];
        \end{axis}
        &
        % Second row, second column (Comfort for N1d_H12h)
        \begin{axis}[
            width=0.45\textwidth,
            height=0.2\textwidth,
            ylabel={Comfort},
            xmin=0, xmax=30,
            xtick={0,5,10,15,20,25,30},
            legend pos=north east,
            grid=major,
            legend style={draw=none},
        ]
            \addplot[
                color=green, thick
            ] table [
                x expr=\coordindex, 
                y=mean_comfort, 
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};
            
            \addplot [
                name path=upper, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_comfort} + sqrt(\thisrow{var_comfort}),
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};

            \addplot [
                name path=lower, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_comfort} - sqrt(\thisrow{var_comfort}),
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};

            \addplot[green!50, fill opacity=0.2] fill between[of=upper and lower];
        \end{axis}
        \\
        % Third row, first column (Total Cost for N1d_H6h)
        \begin{axis}[
            width=0.45\textwidth,
            height=0.2\textwidth,
            xlabel={Learning iteration},
            ylabel={Total cost},
            xmin=0, xmax=30,
            xtick={0,5,10,15,20,25,30},
            legend pos=north east,
            grid=major,
            legend style={draw=none},
        ]
            \addplot[
                color=purple, thick
            ] table [
                x expr=\coordindex, 
                y=mean_total, 
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};
            
            \addplot [
                name path=upper, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_total} + sqrt(\thisrow{var_total}),
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};

            \addplot [
                name path=lower, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_total} - sqrt(\thisrow{var_total}),
                col sep=comma
            ] {Figures/house/N1d_H6h/data.csv};

            \addplot[purple!50, fill opacity=0.2] fill between[of=upper and lower];
        \end{axis}
        &
        % Third row, second column (Total Cost for N1d_H12h)
        \begin{axis}[
            width=0.45\textwidth,
            height=0.2\textwidth,
            xlabel={Learning iteration},
            ylabel={Total cost},
            xmin=0, xmax=30,
            xtick={0,5,10,15,20,25,30},
            legend pos=north east,
            grid=major,
            legend style={draw=none},
        ]
            \addplot[
                color=purple, thick
            ] table [
                x expr=\coordindex, 
                y=mean_total, 
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};
            
            \addplot [
                name path=upper, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_total} + sqrt(\thisrow{var_total}),
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};

            \addplot [
                name path=lower, draw=none
            ] table [
                x expr=\coordindex, 
                y expr=\thisrow{mean_total} - sqrt(\thisrow{var_total}),
                col sep=comma
            ] {Figures/house/N1d_H12h/data.csv};

            \addplot[purple!50, fill opacity=0.2] fill between[of=upper and lower];
        \end{axis}
        \\
    };
\end{tikzpicture}


